Principal Word Vectors

We generalize principal component analysis for embedding words into a vector space. The generalization is made in two major levels. The first is to generalize the concept of the corpus as a counting process which is defined by three key elements vocabulary set, feature (annotation) set, and context. This generalization enables the principal word embedding method to generate word vectors with regard to different types of contexts and different types of annotations provided for a corpus. The second is to generalize the transformation step used in most of the word embedding methods. To this end, we define two levels of transformations. The first is a quadratic transformation, which accounts for different types of weighting over the vocabulary units and contextual features. Second is an adaptive non-linear transformation, which reshapes the data distribution to be meaningful to principal component analysis. The effect of these generalizations on the word vectors is intrinsically studied with regard to the spread and the discriminability of the word vectors. We also provide an extrinsic evaluation of the contribution of the principal word vectors on a word similarity benchmark and the task of dependency parsing. Our experiments are finalized by a comparison between the principal word vectors and other sets of word vectors generated with popular word embedding methods. The results obtained from our intrinsic evaluation metrics show that the spread and the discriminability of the principal word vectors are higher than that of other word embedding methods. The results obtained from the extrinsic evaluation metrics show that the principal word vectors are better than some of the word embedding methods and on par with popular methods of word embedding.

==> acc_neighbourhood.tex <==
\begin{figure}[htp]

  \begin{center}
    \subfloat[]{\scalebox{0.57} {
      \input{neighbourhood_mean_sim_rank.tex}
      \label{fig:neighbourhood_mean_sim_rank}
      }
    }
    %
    \hfill
    %
    \subfloat[]{\scalebox{0.57} {
      \input{lda_pos_neighbourhood.tex}
      \label{fig:lda_pos_neighbourhood}
      }
    }
    %\hspace{0.2\textwidth} %\hfill
    \hfill
    \subfloat[]{\scalebox{0.57} {
      \input{lda_ner_neighbourhood.tex}
      \label{fig:lda_ner_neighbourhood}
      }
    }
  \end{center}
  \caption{The performance of principal word vectors on (a) word similarity tasks, (b) part-of-speech tagging, and (c) named entity recognition. The word vectors are generated with neighbourhood context with different values of $\tau$. The red lines are the baseline obtained with randomly generated word vectors.}

\end{figure}



==> acc_union.tex <==
\begin{figure}[htp]

  \begin{center}
    \subfloat[]{\scalebox{0.57} {
      \input{union_mean_sim_rank.tex}
      \label{fig:union_mean_sim_rank}
      }
    }
    %
    \hfill
    %
    \subfloat[]{\scalebox{0.57} {
      \input{lda_pos_union.tex}
      \label{fig:lda_pos_union}
      }
    }
    %\hspace{0.2\textwidth} %\hfill
    \hfill
    \subfloat[]{\scalebox{0.57} {
      \input{lda_ner_union.tex}
      \label{fig:lda_ner_union}
      }
    }
  \end{center}
  \caption{The performance of principal word vectors on (a) word similarity tasks, (b) part-of-speech tagging, and (c) named entity recognition. The word vectors are generated with union context combination approach with different values of $k$. The red lines are the baseline obtained with randomly generated word vectors.}
  \label{fig:acc_union}

\end{figure}



==> acc_window.tex <==
\begin{figure}[htp]

  \begin{center}
    \subfloat[]{\scalebox{0.6} {
      \input{window_based_mean_sim_rank.tex}
      \label{fig:window-based_mean_sim_rank}
      }
    }
%
    \hfill
%
    \subfloat[]{\scalebox{0.6} {
      \input{lda_pos_window.tex}
      \label{fig:lda_pos_window}
      }
    }
%
    \hfill
%
    \subfloat[]{\scalebox{0.6} {
      \input{lda_ner_window.tex}
      \label{fig:lda_ner_window}
      }
    }
  \end{center}
  \caption{The performance of principal word vectors on (a) word similarity tasks, (b) part-of-speech tagging, and (c) named entity recognition. The word vectors are generated with window-based context with different values of $k$. The red lines are the baseline obtained with randomly generated word vectors.}

\end{figure}



==> best_fisher.tex <==
\begin{figure}[htp]
  \begin{center}
    \subfloat[]{\scalebox{0.80} {
      \input{word_form_best_pos_fisher.tex}
      \label{subfig:word_form_best_pos_fisher}
      }
    }
    %
    \hfill
    %
    \subfloat[]{\scalebox{0.80} {
      \input{pos_best_pos_fisher.tex}
      \label{subfig:pos_best_pos_fisher}
      }
    }
   %%
   \vfill
   %
   \subfloat[]{\scalebox{0.80} {
      \input{word_form_best_ner_fisher.tex}
      \label{subfig:word_form_best_ner_fisher}
      }
    }
   %
   \hfill
   %
   \subfloat[]{\scalebox{0.80} {
     \input{pos_best_ner_fisher.tex}
      \label{subfig:pos_best_ner_fisher}
      }
   }
  \end{center}
  \caption{The best values of fisher discriminant ratio (FDR) obtained from the principal word vectors with regard to word's part of speech tags (top) and named entities (bottom). The word vectors are extracted with two types of contetxual feature sets, word forms (left) and universal part-of-tags (right).}
  \label{fig:best_fisher}
\end{figure}



==> cooc.tex <==
\section{Co-occurrence Matrix}
\label{sec:cooccurrence_matrix}

%We define a \emph{context} in a corpus as a text region formed by a set of words whose presence can be attributed to an abstract unit called \emph{context unit}.
%We associate each context unit with a real-valued random variable that measures the membership degree of words in the context formed by the context unit.
%We will refer to this random variable as \emph{context variable}. 

We define a \emph{context} as a text region in a corpus with a certain type of connection between the elements of the region. 
Some examples of context are the syntactically or semantically connected words in a corpus such as a paragraph, a sentence, a phrase, or just a sequence of words in a sentence that start with word \emph{the}. 
Each context can be associated with a real-valued random variable that measures the extent to which a word belongs to the context.  
We will refer to this random variable as \emph{context variable}. 

Suppose that $\mathscr{C}=(C_1, \dots, C_M)^T$ is a vector of $M$ context variables, then each occurrence of a word in a corpus can be modelled by an $M$ dimensional vector that describes the word from $M$ different perspectives in terms of being in the contexts. 
We will refer to this vectors as \emph{local context-word vector} since it gives a local description about the occurrence of the word. 
As opposed to the local context-word vector, the \emph{global context-word vector} provides a global description over all occurrences of the words in a corpus. 
The global context-word vector of a word can be computed by accumulating all local context-word vectors associated with the word in a corpus. 
Given the corpus $E = (e_1, \dots, e_T)$, the vocabulary list $\mathscr{V}=(w_1,\dots,w_N)$, and the list of context variables $\mathscr{C}=(C_1, \dots, C_M)^T$, the $M \times N$ matrix $\mathcal{C}$ formed by the population of $N$ global context-word vectors is called a co-occurrence matrix and is computed as below:
\begin{equation}
  \mathcal{C} = V\Delta^T
  \label{eq:cooc_matrix}
\end{equation}
where the $t$th column of the $M \times T$ matrix $V$ is the local context-word vector associated with $e_t$ in $E$, and the $t$th column of the $N \times T$ matrix $\Delta$ is a unit sized indicator vectors with all elements equal to zero except for the $j$th element indicating the word $e_t$ in the vocabulary list $\mathscr{V}$, \ie $w_j = e_t$. 

%Different types of context units and membership functions have been used in the literature resulting in two major types of context:
%\begin{itemize}
%  \item window-based context
%  \item syntax-based context
%\end{itemize}
%A window-based context is a sequence of words (or sub-words) associated with the context unit. 


==> cooc2.tex <==
\section{Co-occurrence Matrix}
\label{sec:cooccurrence_matrix}

A co-occurrence matrix shows the frequency of seeing word pairs in the same context.
Context is basically a text region whose elements are in a certain type of connection to each other. 
For example, a set of words with a dependency relation between them  can be seen as a context.

A co-occurrence matrix computed from a corpus shows the frequency of seeing a set of words forming the corpus in different contexts formed in the corpus. 
The context of a word is basically defined as a text region in the corpus whose elements are in a certain type of connection with the word.  
We define the contextual feature of a word as the features associated with the context's elements.
For example, the context of a word can be its immediate parent in a dependency tree and its contextual features can be the syntactic and the morphological features of the parent word. 

Denoting $V = \{v_1, \dots, v_n\}$ as a vocabulary, $E = \{e_1, \dots, e_T\}$ as a corpus with the vocabulary lookup function $L:E\to V$, and $C=\{c_1, \dots, c_m\}$ as the set of contextual features formed in $E$, 
we associate each contextual feature $c_i\in C$ with a Bernoulli variable $\mathbf{c}_i(e_t)$, called \emph{context variable}, whose value for the given word $e_t\in E$ is $1$ if and only if the contextual feature $c_i\in C$ is seen in the context of $e_t\in E$.
Denoting $\mathbf{C}=(\mathbf{c}_1(e_t), \dots, \mathbf{c}_m(e_t))^T$ as a vector of context variables, each occurrence of word $e_t\in E$ is represented by an $m$ dimensional binary vector $\mathcal{v}_{t}$, where $\mathcal{v}_{t}(i)=\mathbf{c}_i(e_t)$.
Using this notation, the $m \times n$ co-occurrence matrix $\mathcal{C}$ is defined as below:
\begin{equation}
  \mathcal{C} = \sum_{t=1}^{T}\mathcal{v}_{t}\delta_{t}^T
  \label{eq:cooc_matrix}
\end{equation}
where $\delta_{t}$ is a unit sized indicator vectors with all elements equal to zero except for the $j$th element which indicates the word $e_t$ in the vocabulary set $V$, \ie $L(e_t) = v_j$.

More complicated co-occurrence matrices can be formed by combining multiple co-occurrence matrices built for the same vocabulary set but different types of contexts. 
The two major types of contexts used in the literature are:
\begin{enumerate*}
  \item window-based context, and
  \item syntax-based context.
\end{enumerate*}
A window-based context is defined by neighbourhood connection between words and a syntax-based context is defined by certain type of syntactic connections between words (\eg dependency connection). 

For example, let's $C$ be a subset of $V$. 
We define the vector of context variable  $\mathbf{C}_d=(\mathbf{c}_1(e_t), \dots, \mathbf{c}_m(e_t))^T$ with $d$ being a positive integer as a neighbourhood context with distance $d$ whose element $\mathbf{c}_i$ ($i=1,\dots,m$) for word $e_t\in E$ are define below:
\begin{equation}
  \mathbf{c}_i(e_t) = 
  \begin{cases}
    1 & L(e_{t-d})=c_i \\
    0 & \mbox{othewise}
  \end{cases}
  \label{eq:neighbourhood_context}
\end{equation}
Basically, $\mathbf{C}_d(i)=\mathbf{c}_i(e_t)$ tells us whether the $d$th word to the left of $e_t\in E$ is $c_i\in C$ or not.

Using $\mathbf{C}_d$ with different values of $d\in D \subset \mathbb{Z}^+$, we define two types of co-occurrence matrices as below over vocabulary $V = \{v_1, \dots, v_n\}$, contextual features $C=\{c_1, \dots, c_m\}$, and corpus $E = \{e_1, \dots, e_T\}$ as below:
\begin{equation}
  \mathcal{C}_D = \sum_{d=1}^{\norm{D}} \mathcal{C}_d
  \label{eq:neighbourhood_cooc}
\end{equation}
, and
\begin{equation}
  \mathcal{C}_D = 
  \begin{pmatrix}
    \mathcal{C}_1^T \dots \mathcal{C}_{\norm{D}}^T
  \end{pmatrix}^T
  \label{eq:stacked_cooc}
\end{equation}
where $\mathcal{C}_d$ ($d=1,\dots,\norm{D}$) is the co-occurrence matrix obtained from the vector of context variable  $\mathbf{C}_d$. 

First is the \emph{weighted window-based context} which is 



Given the vocabulary set $V = \{v_1, \dots, v_n\}$ forming the corpus $E = \{e_1, \dots, e_T\}$ with the vocabulary lookup function $L:E\to V$,  we define $C=\{c_1, \dots, c_m\}$ as the set of all contextual features associated with all contexts that are formed in $E$ for words in $V$. 
Each contextual feature $c_i\in C$ ($i=1\dots m$) can be associated with a real-valued random variable $\mathbf{c}_i$ that measures the association degree between a word and the contextual feature $c_i$.  
We will refer to this random variable as \emph{context variable}. 

Suppose that $\mathbf{C}=(\mathbf{c}_1, \dots, \mathbf{c_m})^T$ is a vector of $m$ context variables, then each occurrence of a word in a corpus can be modelled by an $m$ dimensional vector whose elements measure the membership degree of the word in the corresponding contexts.
We will refer to this vectors as \emph{local context-word vector} since it gives a description about the local occurrence of the word. 
As opposed to the local context-word vector, the \emph{global context-word vector} provides a global description over all occurrences of the words in a corpus. 
The global context-word vector of a word can be computed by accumulating all local context-word vectors associated with the word in a corpus. 
The $m \times n$ matrix $\mathcal{C}$ formed by the population of $n$ global context-word vectors is called a co-occurrence matrix and is computed as below:
\begin{equation}
  \mathcal{C} = \sum_{t=1}^{T}\mathcal{v}_{t}\delta_{t}^T
  \label{eq:cooc_matrix}
\end{equation}
where $\mathcal{v}_{t}$ is the local context-word vector associated with $e_t\in E$, and $\delta_{t}$ is a unit sized indicator vectors with all elements equal to zero except for the $j$th element indicating the word $e_t$ in the vocabulary set $V$, \ie $L(e_t) = v_j$. 

Different types of contexts and contextual features used in the literature 


==> eigen_summary_1.tex <==
\begin{figure}
  \begin{center} 
    \subfloat[]{\scalebox{0.6} {
        \label{subfig:word_form_generalized_variance}
        \input{word_form_generalized_variance.tex}
      }
    }
    %\hfill
    \hspace{0.2\textwidth} %\hfill
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \subfloat[]{\scalebox{0.6} {
        \label{subfig:word_form_best_eigen_spectrum}
        \input{best_eigenspectrum.tex}
      }
    }
    %\hfill
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    %\subfloat[]{\scalebox{0.6} {
    %    \label{subfig:symmetric_window_eigenvalue}
    %    \input{symmetric_window_context_eigval.tex}
    %  }
    %}
  \end{center}
  \caption{The summarization of generalized variance and eigen spectrums obtained from different context functions. (a) is the generalized variance of principal word vectors with respect to the context parameter $x$ which refers to $\tau$ for neighbourhood context and $k$ for other types of context. (b) is the spectrum of eigenvalues with largest value of generalized variance. The neighbourhood refers to the values obtained from both positive and negative values of $\tau$. The \emph{asym window} and \emph{asym union} refer to both backward and forward variants of the window-based and union context functions.}
  \label{fig:eigen_summary_word_form}
\end{figure}



==> feature_eigen_and_variance.tex <==
\begin{figure}
  \begin{center} 
    \subfloat[]{\scalebox{0.6} {
        \label{subfig:feature_eigen}
        \input{feature_eigenvalues.tex}
      }
    }
%    \hspace{0.2\textwidth} %\hfill
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%    \subfloat[]{\scalebox{0.6} {
%         \label{subfig:feature_gen_variance}
%         \input{feature_variance.tex}
%       }
%    }
    %\hfill
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    %\subfloat[]{\scalebox{0.6} {
    %     \label{subfig:dependency_eigenvalue}
    %     \input{dependency_context_eigenval.tex}
    %   }
    %}
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \end{center}
  \caption{}  
  \label{fig:feat_eigen_variance}
\end{figure}



==> fisher_neighbourhood.tex <==
\begin{figure}[htp]

  \begin{center}
   \subfloat[]{\scalebox{0.57} {
      \input{fisher_pos_neighbourhood.tex}
      \label{fig:fisher_pos_neighbourhood}
      }
    }
    %\hspace{0.2\textwidth} %\hfill
    \hfill
    \subfloat[]{\scalebox{0.57} {
      \input{fisher_ner_neighbourhood.tex}
      \label{fig:fisher_ner_neighbourhood}
      }
    }
  \end{center}
  \caption{The performance of principal word vectors on (a) word similarity tasks, (b) part-of-speech tagging, and (c) named entity recognition. The word vectors are generated with neighbourhood context with different values of $\tau$. The red lines are the baseline obtained with randomly generated word vectors.}

\end{figure}



==> fisher_union.tex <==
\begin{figure}[htp]

  \begin{center}
    \subfloat[]{\scalebox{0.57} {
      \input{fisher_pos_union.tex}
      \label{fig:fisher_pos_union}
      }
    }
    %\hspace{0.2\textwidth} %\hfill
    \hfill
    \subfloat[]{\scalebox{0.57} {
      \input{fisher_ner_union.tex}
      \label{fig:fisher_ner_union}
      }
    }
  \end{center}
  \caption{The performance of principal word vectors on (a) word similarity tasks, (b) part-of-speech tagging, and (c) named entity recognition. The word vectors are generated with union context combination approach with different values of $k$. The red lines are the baseline obtained with randomly generated word vectors.}
  \label{fig:acc_union}

\end{figure}



==> fisher_window.tex <==
\begin{figure}[htp]
  \begin{center}
    \subfloat[]{\scalebox{0.6} {
      \input{fisher_pos_window.tex}
      \label{fig:fisher_pos_window}
      }
    }
%
    \hfill
%
    \subfloat[]{\scalebox{0.6} {
      \input{fisher_ner_window.tex}
      \label{fig:fisher_ner_window}
      }
    }
  \end{center}
  \caption{The performance of principal word vectors on (a) word similarity tasks, (b) part-of-speech tagging, and (c) named entity recognition. The word vectors are generated with window-based context with different values of $k$. The red lines are the baseline obtained with randomly generated word vectors.}

\end{figure}



==> generalized_variance.tex <==
\begin{figure}[htp]
  \begin{center}
    \subfloat[]{\scalebox{0.80} {
      \input{word_form_generalized_variance.tex}
      \label{subfig:word_form_generalized_variance}
      }
    }
    %
    \hfill
    %
    \subfloat[]{\scalebox{0.80} {
      \input{pos_generalized_variance}
      \label{subfig:pos_generalized_variance}
      }
    }
  \end{center}
  \caption{The generalized varaiance of principal word vectors generated with different types of feature variables. The feature variables are built with different types of context functions and (a) word forms, and (b) universal part-of-speech tags as their contextual feaures.}
  \label{fig:best_fisher}
\end{figure}



==> lda_acc_union.tex <==
\begin{figure}[htp]

  \begin{center}
    \subfloat[]{\scalebox{0.6} {
      \input{lda_pos_union.tex}
      \label{fig:lda_pos_union}
      }
    }
%
    \hspace{0.2\textwidth} %\hfill
%
    \subfloat[]{\scalebox{0.6} {
      \input{lda_ner_union.tex}
      \label{fig:lda_ner_union}
      }
    }
  \end{center}

\end{figure}



==> lev_diagram.tex <==
\begin{figure}
  \begin{center} 
    \input{lev_diag.tex}
  \end{center}
  \caption{}
  \label{fig:lev_diag}
\end{figure}



==> literature_review.tex <==
\section{Literature Review}
\label{sec:lit_review}



The methods to perform a principal component analysis are:
\begin{itemize}


==> neighbourhood_eigenvalues.tex <==
\begin{figure}
  \begin{center} 
    \subfloat[]{\scalebox{0.6} {
        \label{subfig:backward_neighbourhood_eigenvalue}
        \input{left_neighbourhood_context_eigval.tex}
      }
    }
    \hspace{0.2\textwidth} %\hfill
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \subfloat[]{\scalebox{0.6} {
         \label{subfig:forward_neighbourhood_eigenvalue}
         \input{right_neighbourhood_context_eigval.tex}
       }
    }
    %\hfill
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    %\subfloat[]{\scalebox{0.6} {
    %     \label{subfig:dependency_eigenvalue}
    %     \input{dependency_context_eigenval.tex}
    %   }
    %}
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \end{center}
  \caption{The spectrum of eigenvalues obtained from covariance matrices of principal word vectors generated with (a) the backward neigbourhood context, and (b) the forward neighbourhood context. The vertical axis is the logarithm of the eigenvalues.}
  \label{fig:eigenval_wordform_neighbourhood}
\end{figure}



==> neighbourhood_sim_rank.tex <==
\begin{figure}[htp]
  \begin{center} 
    \subfloat[]{\scalebox{1} {
      \label{subfig:backward_neighbourhood_sim_rank}
      \input{left_neighbourhood_context_sim_rank.tex}
    }
  }
  \vfill
  \subfloat[]{\scalebox{1} {
      \label{subfig:forward_neighbourhood_sim_rank}
      \input{right_neighbourhood_context_sim_rank.tex}
    }
  }
  \end{center}

  \caption{Word similarity task: (a) backward neighbourhood context, and (b) forward neighbourhood context}
  \label{fig:sim_task_wordform_neighbourhood}
\end{figure}



==> pca1.tex <==
\section{Principal Component Analysis}
\label{sec:pca}
Principal component analysis (PCA) is a method to study the structure of a data matrix. 
PCA is studied from different views which are rooted in the way that the data matrix is seen \cite{jolliffe2002principal}. 
In a geometric view, the data are seen as vectors in an Euclidean space spanned by the column or row vectors in the data matrix. 
In a statistical view, the data matrix is seen as a sample from a multivariate distribution.  
%The fixed effect model for PCA \cite{} and the probabilistic PCA \cite{} generalizes statistical view by adding a noise parameter to it. 
%A detailed study about different models of PCA is done by \newcite{}. 

In this paper, we focus on the statistical view of PCA since it is more relevant to the way that we model a co-occurrence matrix. 
PCA, in an statistical view, deals with the study of the structure of covariance between a vector of random variables $\mathbf{X}=(\mathbf{x}_1, \dots, \mathbf{x}_m)^T$. 
It looks for a vector of independent latent variables $\mathbf{Y}=(\mathbf{y}_1, \dots \mathbf{y}_k)$ ($k \ll m$), inferred from the original variables, whose variances under projection of original variables are maximal. 
The latent variables, called \emph{principal components}, are linear functions of original variables, $\mathbf{Y}=A^T (\mathbf{X} - \mathbf{E[\mathbf{X}]})$, where $\mathbf{E[\mathbf{X}]}$ is the expected vector of the random variables, and the $m \times k$ matrix $A=[A_1 \dots A_k]$ is the $k$ dominant eigenvectors of the covariance matrix $S=\mathbf{E}[(\mathbf{X}-\mathbf{E}[\mathbf{X}])(\mathbf{X}-\mathbf{E}[\mathbf{X}])^T]$, \ie $SA_j = \lambda_j A_j$.
It can be shown that the variance of each random variable $\mathbf{y}_j$ ($j=1\dots k$) is equal to the eigenvalue $\lambda_j$ associated with $A_j$.

\ALG{alg:standard_pca} shows how to estimate the principal components $\mathbf{Y}$ from an $m \times n$ sample matrix $X$ drawn from the random vector $\mathbf{X}=(\mathbf{x}_1, \dots, \mathbf{x}_m)^T$. 
\begin{algorithm}
  \begin{algorithmic}
    \Procedure{PCA}{$X,k$} 
      \State Estimate the sample mean vector $\overline{X} \gets \frac{1}{n}X\mathbf{1}_n$
      \State Estimate the covariance matrix $S \gets \frac{1}{n-1}(X-\overline{X}\mathbf{1}_n^T) (X-\overline{X}\mathbf{1}_n^T)^T$
      \State Form the $m \times k$ matrix $A$ by $k$ dominant eigenvectors of $S$ such that $SA_j = \lambda_j A_j$
      \State Form the $k$ dimensional principal components $Y \gets A^T (X - \bar{X}\mathbf{1}_n^T)$
      \State \textbf{return} $Y$
    \EndProcedure
  \end{algorithmic}
  \caption{The $k$-dimensional principal component analysis of the $m \times n$ sample matrix $X$. $\mathbf{1}_n$ is the vector of $n$ ones.}
\label{alg:standard_pca}
\end{algorithm}

The eigenvectors $A$ in \ALG{alg:standard_pca} can be efficiently computed by singular value decomposition of the \emph{mean-centred} sample matrix $\mathcal{X} = X - \overline{X}\mathbf{1}_n^T$. 
The left singular vectors of $\mathcal{X}$ are the eigenvectors of the covariance matrix $S$, and the singular values are equal to $\sqrt{(n-1)\lambda}$, where $\lambda$ is vector of eigenvalues of $S$.  
Using the singular value decomposition of $\mathcal{X} = U\Sigma V^T$, the principal components can be efficiently computed by $Y=U^T\mathcal{X}$, or equivalently by $Y=\Sigma V^T$. 
\ALG{alg:svd_pca} summarizes how to compute the top $k$ principal components of the sample matrix $X$ using singular value decomposition.
\begin{algorithm}
  \begin{algorithmic}
    \Procedure{PCA}{$X,k$} 
      \State Estimate the sample mean vector $\overline{X} \gets \frac{1}{n}X\mathbf{1}_n$
      \State Form the mean-centred date matrix $\mathcal{X} \gets X - \overline{X}\mathbf{1}_n^T$ and compute its singular value decomposition $\mathcal{X}=U\Sigma V^T$
      \State Form the $k$ dimensional principal components $Y \gets \Sigma V^T$
      \State \textbf{return} $Y$
    \EndProcedure
  \end{algorithmic}
  \caption{The $k$-dimensional principal component analysis of the $m \times n$ sample matrix $X$ using singular value decomposition. $\mathbf{1}_n$ is the vector of $N$ ones.}
\label{alg:svd_pca}
\end{algorithm}

\ALG{alg:svd_pca} can be generalized in various ways \cite{jolliffe2002principal,gpca2016}.
One way of generalization is to centre the data around an arbitrary vector $E$ instead of the sample mean vector $\mathbf{E}[\mathbf{X}]$. 
For example, in terms of statistics, $E$ can be any measures of central tendency such as mode and median. 
Another generalization is to add an $m \times m$ metric matrix $\Phi$, and an $n \times n$ weight matrix $\Omega$ to the classical definition of PCA. 
These matrices provide for using a priori knowledge in the classical PCA. 
The metric matrix $\Phi$ is defined over the random variables and allows of weighting the random variables. 
The weight matrix $\Omega$, which is usually a diagonal matrix, is used to weight the observations. 
It is also quite common to transform the data before performing the singular value decomposition. 
This adds a degree of non-linearity to the classical PCA and is helpful when the non-linear relationships between the variables are of interest.  

\ALG{alg:gpca} shows a generalized version of PCA with respect to the parameters mentioned above. 
The inputs to GPCA are:
\begin{enumerate}
  \item the $m \times n$ matrix of \emph{transformed data} sampled from the vector of random variables,
  \item the $m$ dimensional vector $E$ around which the date is centred, 
  \item the $m \times m$ metric matrix $\Phi$, and 
  \item The $n \times n$ weight matrix $\Omega$.
\end{enumerate}
If $\Omega$ is the identity matrix and $E$ is the vector of expected values over the random variables in $\mathbf{X}=(\mathbf{x}_1, \dots, \mathbf{x}_m)^T$ then GPCA reduces to the classical PCA over
\begin {itemize}
  \item covariance matrix if $\Phi$ is the identity matrix, and
  \item correlation matrix if $\Phi$ is a diagonal matrix with $\frac{1}{\sigma_{i,i}}$ on its main diagonal, where $\sigma_{i,i}$ is the variance of random variable $\mathbf{x}_i$.
\end{itemize}
\begin{algorithm}
  \begin{algorithmic}
    \Procedure{GPCA}{$X,E,\Phi,\Omega,k$} 
      \State Form $\mathcal{X} \gets \Phi (X - E\mathbf{1}_n^T) \Omega$ and compute its singular value decomposition $\mathcal{X}=U\Sigma V^T$
      \State Form the $k$ dimensional principal components $Y \gets \Sigma V^T$
      \State \textbf{return} $Y$
    \EndProcedure
  \end{algorithmic}
  \caption{Generalized principal component analysis.}
\label{alg:gpca}
\end{algorithm}

A drawback of using \ALG{alg:svd_pca} and \ALG{alg:gpca} on a large sparse matrix such as a co-occurrence matrix is that the algorithms cannot take the advantage of sparsity in the input matrix. 
It is because the matrix $\mathcal{X}$ is both algorithms is a dense matrix and needs huge amount of memory and CPU time to be processed by the subsequent SVD step. 
In \SEC{sec:svd}, we propose an efficient algorithm to estimate the singular value decomposition $\mathcal{X}=U\Sigma V^T$ from the input matrix $X$ and the sample mean vector $\overline{X}$ without explicitly forming the dense matrix $\mathcal{X}$. 
The algorithm enable us to take the advantage of sparsity in the input matrix to estimate the principal components of large sparse matrices. 


==> pos_fisher.tex <==
\begin{figure}[htp]
  \begin{center}
    \subfloat[]{\scalebox{0.57} {
      \input{pos_pos_neighbourhood_fisher.tex}
      \label{subfig:pos_pos_neighbourhood_fisher}
      }
    }
    %
    \hfill
    %
    \subfloat[]{\scalebox{0.57} {
      \input{pos_pos_window-based_fisher.tex}
      \label{subfig:pos_pos_window-based_fisher}
      }
    }
    %\hspace{0.2\textwidth} %\hfill
    \hfill
    \subfloat[]{\scalebox{0.57} {
      \input{pos_pos_union_fisher.tex}
      \label{subfig:pos_pos_union_fisher}
      }
    }
    %
    \vfill
    %
    \subfloat[]{\scalebox{0.57} {
      \input{pos_ner_neighbourhood_fisher.tex}
      \label{subfig:pos_ner_neighbourhood_fisher}
      }
    }
    %
    \hfill
    %
    \subfloat[]{\scalebox{0.57} {
      \input{pos_ner_window-based_fisher.tex}
      \label{subfig:pos_ner_window-based_fisher}
      }
    }
    %\hspace{0.2\textwidth} %\hfill
    \hfill
    \subfloat[]{\scalebox{0.57} {
      \input{pos_ner_union_fisher.tex}
      \label{subfig:pos_ner_union_fisher}
      }
    }
  \end{center}
  \caption{Fisher discriminant ratio (FDR) of principal word vectors with regard to word's part of speech tags (top) and named entities (bottom). The word vectors are extracted different types of features variables formed with uniforsal part-of-speech tags and (a,d) neighbourhood context, (b,e) window-based context, (c,f) union context.}
  \label{fig:pos_fisher}
\end{figure}



==> q.tex <==
\begin{figure}
  \begin{center} 
    \subfloat[]{\scalebox{0.8} {
        \label{subfig:q_pos}
        \input{q_pos.tex}
      }
    }
    \hfill
    \subfloat[]{\scalebox{0.8} {
        \label{subfig:q_ner}
        \input{q_ner.tex}
      }
    }
    \hfill
    %\hspace{0.2\textwidth} %\hfill
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \subfloat[]{\scalebox{0.8} {
        \label{subfig:q_generalized_variance}
        \input{q_generalized_variance.tex}
      }
    }
  \end{center}
  \caption{}
  \label{fig:q}
\end{figure}



==> randomness.tex <==
\subsection{The Effect of Randomness}
As elaborated in \SEC{} and \SEC{}, principal word vectors might be affected by two sources of randomness. 
First is the random sampling in Line~\ref{} at \ALG{} and second is the random sampling used to estimate the entropy of the mixture of principal word vectors in \EQ{}. 
In order to see how principal word vector are affected by these sources of randomness, we run the following two experiments $10$ times and study the spread and the discriminability of word vectors at each trial.
In the first series of experiments, we focus on the effect of the randomness in \ALG{}. 
To this end, we disable the effect of the second source of randomness through using the identity transformation function. 
In the second series of experiments, we use the transformation function tuned with with maximum entropy in ....




==> references.tex <==
\begin{thebibliography}{45}
\expandafter\ifx\csname natexlab\endcsname\relax\def\natexlab#1{#1}\fi

\bibitem[{Basirat and Nivre(2017)}]{basirat-nivre:2017:NoDaLiDa}
Basirat, Ali and Joakim Nivre. 2017.
\newblock Real-valued syntactic word vectors (rsv) for greedy neural dependency
  parsing.
\newblock In \emph{Proceedings of the 21th Nordic Conference on Computational
  Linguistics (NoDaLiDa)}, pages 20--28, Association for Computational
  Linguistics, Gothenburg, Sweden.

\bibitem[{Berg-Kirkpatrick, Burkett, and
  Klein(2012)}]{Berg-Kirkpatrick:2012:EIS:2390948.2391058}
Berg-Kirkpatrick, Taylor, David Burkett, and Dan Klein. 2012.
\newblock An empirical investigation of statistical significance in nlp.
\newblock In \emph{Proceedings of the 2012 Joint Conference on Empirical
  Methods in Natural Language Processing and Computational Natural Language
  Learning}, EMNLP-CoNLL '12, pages 995--1005, Association for Computational
  Linguistics, Stroudsburg, PA, USA.

\bibitem[{Blei, Ng, and Jordan(2003)}]{blei2003latent}
Blei, David~M, Andrew~Y Ng, and Michael~I Jordan. 2003.
\newblock Latent dirichlet allocation.
\newblock \emph{Journal of machine Learning research}, 3(Jan):993--1022.

\bibitem[{Chen and Manning(2014)}]{chen14}
Chen, Danqi and Christopher Manning. 2014.
\newblock A fast and accurate dependency parser using neural networks.
\newblock In \emph{Proceedings of the 2014 Conference on Empirical Methods in
  Natural Language Processing (EMNLP)}, pages 740--750.

\bibitem[{Church and Hanks(1990)}]{church1990word}
Church, Kenneth~Ward and Patrick Hanks. 1990.
\newblock Word association norms, mutual information, and lexicography.
\newblock \emph{Computational linguistics}, 16(1):22--29.

\bibitem[{Collobert et~al.(2011)Collobert, Weston, Bottou, Karlen, Kavukcuoglu,
  and Kuksa}]{collobert2011natural}
Collobert, Ronan, Jason Weston, L{\'e}on Bottou, Michael Karlen, Koray
  Kavukcuoglu, and Pavel Kuksa. 2011.
\newblock Natural language processing (almost) from scratch.
\newblock \emph{The Journal of Machine Learning Research}, 12:2493--2537.

\bibitem[{Craddock(1969)}]{craddock69}
Craddock, C.~R., J. M.;~Flood. 1969.
\newblock Eigenvectors for representing the 500 mb. geopotential surface over
  the northern hemisphere.
\newblock \emph{Quarterly Journal of the Royal Meteorological Society},
  95:576--593.

\bibitem[{Dahl, Adams, and Larochelle(2012)}]{ICML2012Dahl_364}
Dahl, George, Ryan Adams, and Hugo Larochelle. 2012.
\newblock Training restricted boltzmann machines on word observations.
\newblock In \emph{Proceedings of the 29th International Conference on Machine
  Learning (ICML-12)}, ICML '12, pages 679--686, Omnipress, New York, NY, USA.

\bibitem[{De~Marneffe and Manning(2010)}]{de2010stanford}
De~Marneffe, Marie-Catherine and Christopher~D Manning. 2010.
\newblock Stanford typed dependencies manual (2008).
\newblock \emph{URL:
  \url{http://nlp.stanford.edu/software/dependencies_manual.pdf}}.

\bibitem[{Dyer et~al.(2015)Dyer, Ballesteros, Ling, Matthews, and
  Smith}]{dyer:2015acl}
Dyer, Chris, Miguel Ballesteros, Wang Ling, Austin Matthews, and Noah~A. Smith.
  2015.
\newblock Transition-based dependeny parsing with stack long short-term memory.
\newblock In \emph{Proceedings of the 53rd Annual Meeting of the Association
  for Computational Linguistics (ACL) and the 7th International Joint
  Conference on Natural Language Processing}, pages 334--343.

\bibitem[{Egghe(2007)}]{ASI:ASI20524}
Egghe, Leo. 2007.
\newblock Untangling herdan's law and heaps' law: Mathematical and informetric
  arguments.
\newblock \emph{Journal of the American Society for Information Science and
  Technology}, 58(5):702--709.

\bibitem[{Faruqui and Dyer(2014)}]{faruqui-2014:SystemDemo}
Faruqui, Manaal and Chris Dyer. 2014.
\newblock Community evaluation and exchange of word vectors at wordvectors.org.
\newblock In \emph{Proceedings of the 52nd Annual Meeting of the Association
  for Computational Linguistics: System Demonstrations}, Association for
  Computational Linguistics, Baltimore, USA.

\bibitem[{Golub and Van~Loan(1996)}]{Golub:MC}
Golub, Gene~H. and Charles~F. Van~Loan. 1996.
\newblock \emph{Matrix Computations}, third edition.
\newblock Johns Hopkins University Press, Baltimore, MD, USA.

\bibitem[{Haji\v{c} and Zeman(2017)}]{K17-3:2017}
Haji\v{c}, Jan and Dan Zeman, editors. 2017.
\newblock \emph{Proceedings of the CoNLL 2017 Shared Task: Multilingual Parsing
  from Raw Text to Universal Dependencies}.
\newblock Association for Computational Linguistics, Vancouver, Canada.

\bibitem[{Halko, Martinsson, and Tropp(2011)}]{Halko2011finding}
Halko, N., P.~G. Martinsson, and J.~A. Tropp. 2011.
\newblock Finding structure with randomness: Probabilistic algorithms for
  constructing approximate matrix decompositions.
\newblock \emph{SIAM Review}, 53(2):217--288.

\bibitem[{Hinton and Salakhutdinov(2006)}]{Hinton504}
Hinton, G.~E. and R.~R. Salakhutdinov. 2006.
\newblock Reducing the dimensionality of data with neural networks.
\newblock \emph{Science}, 313(5786):504--507.

\bibitem[{Hofmann(1999)}]{hofmann1999probabilistic}
Hofmann, Thomas. 1999.
\newblock Probabilistic latent semantic indexing.
\newblock In \emph{Proceedings of the 22nd annual international ACM SIGIR
  conference on Research and development in information retrieval}, pages
  50--57, ACM.

\bibitem[{Jolliffe(2002)}]{jolliffe2002principal}
Jolliffe, I.T. 2002.
\newblock \emph{Principal Component Analysis}.
\newblock Springer Series in Statistics. Springer-Verlag.

\bibitem[{Kiela and Clark(2014)}]{kiela2014systematic}
Kiela, Douwe and Stephen Clark. 2014.
\newblock A systematic study of semantic vector space model parameters.
\newblock In \emph{Proceedings of the 2nd Workshop on Continuous Vector Space
  Models and their Compositionality (CVSC) at Conference of the European
  Chapter of the Association for Computational Linguistics (EACL)}, pages
  21--30.

\bibitem[{Landauer and Dumais(1997)}]{landauer1997solution}
Landauer, Thomas~K and Susan~T Dumais. 1997.
\newblock A solution to {P}lato's problem: The latent semantic analysis theory
  of acquisition, induction, and representation of knowledge.
\newblock \emph{Psychological review}, 104(2):211.

\bibitem[{Lebret and Collobert(2014)}]{lebret-collobert:2014:EACL}
Lebret, R\'{e}mi and Ronan Collobert. 2014.
\newblock Word embeddings through hellinger pca.
\newblock In \emph{Proceedings of the 14th Conference of the European Chapter
  of the Association for Computational Linguistics (EACL)}, pages 482--490,
  Association for Computational Linguistics, Gothenburg, Sweden.

\bibitem[{Lebret and Collobert(2015)}]{DBLP:conf/cicling/LebretC15}
Lebret, R{\'{e}}mi and Ronan Collobert. 2015.
\newblock Rehabilitation of count-based models for word vector representations.
\newblock In \emph{Proceedings of the 16th International Conference on
  Computational Linguistics and Intelligent Text Processing, CICLing}, pages
  417--429, Cairo, Egypt.

\bibitem[{LeCun et~al.(2012)LeCun, Bottou, Orr, and
  M{\"u}ller}]{lecun2012efficient}
LeCun, Yann~A, L{\'e}on Bottou, Genevieve~B Orr, and Klaus-Robert M{\"u}ller.
  2012.
\newblock Efficient backprop.
\newblock In \emph{Neural networks: Tricks of the trade}. Springer, pages
  9--48.

\bibitem[{Levy and Goldberg(2014{\natexlab{a}})}]{levy-goldberg:2014:P14-2}
Levy, Omer and Yoav Goldberg. 2014{\natexlab{a}}.
\newblock Dependency-based word embeddings.
\newblock In \emph{Proceedings of the 52nd Annual Meeting of the Association
  for Computational Linguistics (Volume 2: Short Papers)}, pages 302--308,
  Association for Computational Linguistics, Baltimore, Maryland.

\bibitem[{Levy and Goldberg(2014{\natexlab{b}})}]{levy2014neural}
Levy, Omer and Yoav Goldberg. 2014{\natexlab{b}}.
\newblock Neural word embedding as implicit matrix factorization.
\newblock In \emph{Advances in neural information processing systems}, pages
  2177--2185.

\bibitem[{Lund and Burgess(1996)}]{lund1996producing}
Lund, Kevin and Curt Burgess. 1996.
\newblock Producing high-dimensional semantic spaces from lexical
  co-occurrence.
\newblock \emph{Behavior Research Methods, Instruments, \& Computers},
  28(2):203--208.

\bibitem[{Marcus, Santorini, and Marcinkiewicz(1993)}]{Marcus93_WSJ}
Marcus, Mitchell~P., Beatrice Santorini, and Mary~Ann Marcinkiewicz. 1993.
\newblock Building a large annotated corpus of {English}: The {Penn} treebank.
\newblock \emph{Computational Linguistics - Special issue on using large
  corpora}, 19(2):313 -- 330.

\bibitem[{Matthews(1981)}]{syntax_book_Matthews}
Matthews, Peter~H. 1981.
\newblock \emph{Syntax}.
\newblock Cambridge Textbooks in Linguistics. Cambridge University Press.

\bibitem[{Melamud and Goldberger(2017)}]{melamud-goldberger:2017:Short}
Melamud, Oren and Jacob Goldberger. 2017.
\newblock Information-theory interpretation of the skip-gram negative-sampling
  objective function.
\newblock In \emph{Proceedings of the 55th Annual Meeting of the Association
  for Computational Linguistics (Volume 2: Short Papers)}, pages 167--171,
  Association for Computational Linguistics, Vancouver, Canada.

\bibitem[{Mikolov et~al.(2013{\natexlab{a}})Mikolov, Chen, Corrado, and
  Dean}]{Mikolov13vector_space}
Mikolov, Tomas, Kai Chen, Greg Corrado, and Jeffrey Dean. 2013{\natexlab{a}}.
\newblock Efficient estimation of word representations in vector space.
\newblock In \emph{Proceedings of Workshop at International Conference on
  Learning Representations (ICLR)}.

\bibitem[{Mikolov et~al.(2013{\natexlab{b}})Mikolov, Sutskever, Chen, Corrado,
  and Dean}]{NIPS2013_5021}
Mikolov, Tomas, Ilya Sutskever, Kai Chen, Greg~S Corrado, and Jeff Dean.
  2013{\natexlab{b}}.
\newblock Distributed representations of words and phrases and their
  compositionality.
\newblock In C.~J.~C. Burges, L.~Bottou, M.~Welling, Z.~Ghahramani, and K.~Q.
  Weinberger, editors, \emph{Advances in Neural Information Processing Systems
  26}. Curran Associates, Inc., pages 3111--3119.

\bibitem[{Nivre(2004)}]{nivre2004incrementality}
Nivre, Joakim. 2004.
\newblock Incrementality in deterministic dependency parsing.
\newblock In \emph{Proceedings of the Workshop on Incremental Parsing: Bringing
  Engineering and Cognition Together}, pages 50--57, Association for
  Computational Linguistics.

\bibitem[{Nivre et~al.(2016)Nivre, de~Marneffe, Ginter, Goldberg, Hajic,
  Manning, McDonald, Petrov, Pyysalo, Silveira et~al.}]{nivre2016universal}
Nivre, Joakim, Marie-Catherine de~Marneffe, Filip Ginter, Yoav Goldberg, Jan
  Hajic, Christopher~D Manning, Ryan McDonald, Slav Petrov, Sampo Pyysalo,
  Natalia Silveira, et~al. 2016.
\newblock Universal dependencies v1: A multilingual treebank collection.
\newblock In \emph{Proceedings of the 10th International Conference on Language
  Resources and Evaluation (LREC 2016)}.

\bibitem[{Pad{\'o} and Lapata(2007)}]{pado2007depssm}
Pad{\'o}, Sebastian and Mirella Lapata. 2007.
\newblock Dependency-based construction of semantic space models.
\newblock \emph{Computational Linguistics}, 33.

\bibitem[{Pennington, Socher, and Manning(2014)}]{pennington2014glove}
Pennington, Jeffrey, Richard Socher, and Christopher~D Manning. 2014.
\newblock Glove: Global vectors for word representation.
\newblock In \emph{Proceedings of the 2014 Conference on Empirical Methods in
  Natural Language Processing (EMNLP)}, volume~14, pages 1532--1543.

\bibitem[{Reed et~al.(2006)Reed, Jiao, Potok, Klump, Elmore, and
  Hurson}]{tf-icf:4041501}
Reed, Joel~W., Yu~Jiao, Thomas~E. Potok, Brian~A. Klump, Mark~T. Elmore, and
  Ali~R. Hurson. 2006.
\newblock Tf-icf: A new term weighting scheme for clustering dynamic data
  streams.
\newblock In \emph{2006 5th International Conference on Machine Learning and
  Applications (ICMLA'06)}, pages 258--263.

\bibitem[{Ren{\'e}~Vidal(2016)}]{gpca2016}
Ren{\'e}~Vidal, S. Shankar~Sastry, Yi~Ma. 2016.
\newblock \emph{Generalized Principal Component Analysis}.
\newblock Interdisciplinary Applied Mathematic. Springer-Verlag.

\bibitem[{Roweis and Saul(2000)}]{Roweis2323LLE}
Roweis, Sam~T. and Lawrence~K. Saul. 2000.
\newblock Nonlinear dimensionality reduction by locally linear embedding.
\newblock \emph{Science}, 290(5500):2323--2326.

\bibitem[{Sahlgren(2006)}]{sahlgren2006word}
Sahlgren, Magnus. 2006.
\newblock \emph{The Word-space model}.
\newblock Ph.D. thesis, Stockholm University.

\bibitem[{Salton and Buckley(1988)}]{salton1988term}
Salton, Gerard and Christopher Buckley. 1988.
\newblock Term-weighting approaches in automatic text retrieval.
\newblock \emph{Information processing \& management}, 24(5):513--523.

\bibitem[{Sch{\"u}tze(1992)}]{schutze1992dimensions}
Sch{\"u}tze, Hinrich. 1992.
\newblock Dimensions of meaning.
\newblock In \emph{Proceedings of the 1992 ACM/IEEE conference on
  Supercomputing}, pages 787--796, IEEE Computer Society Press.

\bibitem[{Straka and Strakov\'{a}(2017)}]{udpipe:2017}
Straka, Milan and Jana Strakov\'{a}. 2017.
\newblock Tokenizing, pos tagging, lemmatizing and parsing ud 2.0 with udpipe.
\newblock In \emph{Proceedings of the CoNLL 2017 Shared Task: Multilingual
  Parsing from Raw Text to Universal Dependencies}, pages 88--99, Association
  for Computational Linguistics, Vancouver, Canada.

\bibitem[{Tjong Kim~Sang and
  De~Meulder(2003)}]{TjongKimSang:2003:ICS:1119176.1119195}
Tjong Kim~Sang, Erik~F. and Fien De~Meulder. 2003.
\newblock Introduction to the conll-2003 shared task: Language-independent
  named entity recognition.
\newblock In \emph{Proceedings of the Seventh Conference on Natural Language
  Learning at HLT-NAACL 2003 - Volume 4}, CONLL '03, pages 142--147,
  Association for Computational Linguistics, Stroudsburg, PA, USA.

\bibitem[{Toutanova et~al.(2003)Toutanova, Klein, Manning, and
  Singer}]{toutanova2003feature}
Toutanova, Kristina, Dan Klein, Christopher~D Manning, and Yoram Singer. 2003.
\newblock Feature-rich part-of-speech tagging with a cyclic dependency network.
\newblock In \emph{Proceedings of the 2003 Conference of the North American
  Chapter of the Association for Computational Linguistics on Human Language
  Technology-Volume 1}, pages 173--180, Association for Computational
  Linguistics.

\bibitem[{Zobel, Heinz, and Williams(2001)}]{Zobel2001Hash}
Zobel, Justin, Steffen Heinz, and Hugh~E. Williams. 2001.
\newblock In-memory hash tables for accumulating text vocabularies.
\newblock \emph{Information Processing Letters}, 80:271--277.

\end{thebibliography}


==> svd_original.tex <==
\subsection{Centred Singular Value Decomposition}
\label{sec:svd}
Any real-valued $m\times n$ matrix $X$ can be decomposed into three matrices as $X = U\Sigma V^T$
where the $m \times m$ matrix $U$ and $n \times n$ matrix $V$ are real-valued orthonormal matrices (\ie $U^TU=I_{m}$ and $V^TV=I_{n}$), and $\Sigma$ is a diagonal $m \times n$ matrix whose diagonal elements are non-negative real values. 

As mentioned before, the set of principal components of a mean centred matrix can be efficiently computed from the singular values and singular vectors of the matrix. 
In this section, we propose a method of singular value decomposition for this aim. 
Denoting $X$ as an $m \times n$ matrix, $E$ as an $m$ dimensional vector, and $\mathbf{1}_n$ as an $n$ dimensional vector of ones,
\ALG{alg:rsvd}, inspired by the randomized matrix factorization method introduced by \namecite{halko2011finding}, 
returns a rank-$k$ approximation of the singular value decomposition of the data matrix $\mathscr{X} = X - E\mathbf{1}_n^T$, whose columns are centred around the vector $E$. 
The algorithm works as follows.
First, it approximates a rank $K$ basis matrix $Q$ ($k<K\ll n$) that captures most of the information in the input matrix $\mathscr{X}$. 
This step can be efficiently done by \ALG{alg:randomized_subspace_iteration}, which will be elaborated in \SEC{subsec:centred_qr}. 
Then the data matrix $\mathscr{X}$ is projected to the space spanned by $Q$, \ie $Y = Q^T\mathscr{X}$, using the distributive property of multiplication over addition, \ie $Y = Q^TX_1 - Q^TE\mathbf{1}_n^T$. 
Finally, the SVD factors of $\mathscr{X}$ are estimated from the $K \times n$ matrix $Y$ in two steps.  
First, the rank-$k$ SVD approximation of $Y$ is computed using a standard method of singular value decomposition, \ie $Y=U_{1}SV^T$ (Line~\ref{alg:rsvd:svd}). 
Then the left singular vectors are updated by $U \leftarrow QU_{1}$ resulting in $USV^T=QY$, which is the rank-$k$ approximation of $\mathscr{X}$ (Line~\ref{alg:rsvd:qu}).
\begin{algorithm}[H]
  \begin{algorithmic}[1]
    \Procedure{Centred-SVD}{$X,E,k,K$} 
      \State Construct the $m \times K$ orthonormal basis matrix $Q$ whose columns form the range of $\mathscr{X} = X - E\mathbf{1}_n^T$
      \State Form $Y \gets Q^TX - Q^TE\mathbf{1}_n^T$   \label{alg:projection}
      \State Compute the singular value decomposition of $Y = U_{1}SV^T$ \label{alg:rsvd:svd}
      \State $U \gets QU_{1}$         \label{alg:rsvd:qu}
      \State \Return $(U, \Sigma, V)$
    \EndProcedure
  \end{algorithmic}
  \caption{Singular value decomposition of $X-E\mathbf{1}_n^T=U\Sigma V^T$.}
\label{alg:rsvd}
\end{algorithm}

Note that in Line~\ref{alg:projection}, instead of applying the product operator on $Q$ and $X-E\mathbf{1}_n^T$, we use $Q^TX_1 - Q^TE\mathbf{1}_n^T$. 
This is because the amount of memory required by the latter approach is significantly smaller than the amount of memory required by the former approach. 
In the former approach, one needs to build the $m\times n$ matrix $X-E\mathbf{1}_n^T$ but in the latter approach we have two $m\times K$ matrices $Q^TX_1$ and $Q^TE\mathbf{1}_n^T$. 
Since $K\ll m$ and in many applications the number of observations $n$ is larger than or equal (or at least comparable) to the number of variables $m$ ($m\le n$), the latter approach is more efficient. 
Moreover, since the matrix $Q^TE\mathbf{1}_n^T$ repeats the column vectors $Q^TE$ in all its columns, instead of building this matrix one can subtract the column vector $Q^TE$ from all columns of $Q^TX_1$ in a loop. 

\subsection{Centred QR Factorization}
\label{subsec:centred_qr}
A basis matrix of a vector space contains a set of linearly independent vectors that span the vector space. 
In this section, we elaborate how to estimate an $m\times K$ basis matrix $Q$ from $n$ vectors sampled from an $m$ dimensional vector space. 
Among the methods proposed by \namecite{halko2011finding}, we found the \emph{randomized subspace iteration} method most appropriate for our research. 
The method is designed for very large matrices with flat singular spectrum. 
Depending on the size of the vocabulary set and the size of the feature set used in a corpus, a sample matrix of contextual word vectors collected from the corpus can be very large. 
As explained in \SEC{}, the spectrum of singular vectors of the sample matrix of the contextual word vector highly depends on the size of feature set. 
A large feature set is expected to result in a very large sample matrix and a very sharp decay in the singular spectrum but a small feature set is expected to result in a relatively smaller sample matrix and a flat singular spectrum. 
We conclude that the algorithm is suitable for processing the sample matrix of contextual word vectors in the sense that the matrix is usually large but not in the sense that the singular spectrum is \emph{always} flat.
Nevertheless, as will be explained later in this section, the algorithm provides a tuning parameter, called $q$, which deals with the singular spectrum of the sample matrix. 
We will show in \SEC{} that in the cases where the singular spectrum decays sharply, satisfactory results can be obtained with $q=0$. 

Given the $m \times n$ input matrix $X$, the algorithm of randomized subspace iteration approximates the basis matrix $Q$ from $B=(XX^T)^qX$, where $q$ is a small integer. 
The matrix $B$ has the same singular vectors as $X$ but with a sharp decay in the singular values which is due to the polynomial growth rate of the singular values of $B$. 
Replacing $X$ with its singular value decomposition (i.e. $X=U\Sigma V^T$), we have $B=U\Sigma^{(2q+1)}V^T$. 
Since $q$ is a positive integer, the effect of the polynomial growth on the top singular values is higher than the others.
So, we can say, $B$ expands the data points in $X$ through increasing the variance along the singular vectors of $X$ and the degree of expansion is dependent on the value of corresponding singular values. 
In other words, the increase rate of the variance along the singular vectors associated with top singular values is higher than the increase rate along the singular vectors associated with smaller singular values. 
This data expansion is useful for the cases where the singular spectrum is flat and the distinction between the singular values is not so clear. 

The randomized subspace iteration has two main steps.
First it forms the $m \times K$ matrix $Y=B\Omega$, where the $m\times n$ matrix $B=(XX^T)^qX$ and the $m \times n$ matrix $X$ is the input matrix, the $n \times K$ matrix $\Omega$ is a Gaussian random matrix, and $K > 0$ and $q\geq 0$ are integers.
%\footnote{We observed in our experiments that the random matrix $\Omega$ does not necessary need to be sampled from the standard Gaussian distribution. 
%We obtained the same reconstruction accuracy $\norm{X-QQ^TX}$ from the basis matrix $Q$ computed by the uniform distribution.}
The random matrix $\Omega$ is used to sample $K$ independent points in the range of $B$ which has the same range as $X$. 
So, the columns of $Y$ are linearly independent random points in the range of $X$. 
By way of illustration, the $i$th element of the $j$th sampled vector, $Y_{(i,j)}$, is the linear combination of the $i$th element of all vectors in $B$ and the random linear coefficients in the $j$th row of $\Omega$, \ie $Y_{(i,j)}=\sum_{k=1}^{n} B_{(i,k)}\Omega_{(k,j)}$.
In the second step, it computes the $m \times K$ basis matrix $Q$ via the $QR$ factorization of $Y=QR$.

The computation of the power matrix $Y=(XX^T)^qX\Omega$ can be highly expensive when $X$ is large. 
In order to perform this computation efficiently, both the power matrix $Y$ and the $QR$ factorization $Y=QR$ are computed jointly 
via repeating two $QR$ factorizations as shown in \ALG{alg:original_randomized_subspace_iteration}.
At the $i$the iteration, the $QR$ factorization in Line~\ref{alg_rsi_first_qr} results in  $\overline{Q}_i\overline{R}_i=X^T(XX^T)^{(i-1)}X\Omega$ and the $QR$ factorization in Line~\ref{alg_rsi_second_qr} results in $Q_iR_i=(XX^T)^iX\Omega$. 
If we use these two factorizations repeatedly, we will have the following factorization of the power matrix $Y$: 
\begin{equation}
  \begin{split}
    Y 
      & = (XX^T)^qX\Omega \\
      & =  Q_{q}(\prod_{i=0}^{q-1} {R_{q-i} \overline{R}_{q-i}}) R_0 \\
  \end{split}
  \label{eq:pow_qr1}
\end{equation}
where $Q_0R_0 = X\Omega$, $\overline{Q}_i\overline{R}_i = X^TQ_{i-1}$ and $Q_iR_i=X\overline{Q}_i$.
\begin{algorithm}[H]
  \caption{Estimating the orthonormal basis matrix $Q$ for the $m \times n$ matrix $X$}
  \label{alg:original_randomized_subspace_iteration}
  \begin{algorithmic}[1]
    \Procedure{Randomized-Subspace-Iteration}{$X,K,q$} 
      \State Draw an $n \times K$ standard Gaussian matrix $\Omega$ 
      \State Form $Y_0 \gets X\Omega$ and compute the QR factorization $Y_0 = Q_0R_0$
      \For {$j\gets1$ \textbf{to} $q$}
        \State Form $\overline{Y}_j \gets X^TQ_{j-1}$ and compute the QR factorization $\overline{Y}_j = \overline{Q}_j\overline{R}_j$ \label{alg_rsi_first_qr}
        \State Form $Y_j \gets X\overline{Q}_{j}$ and compute the QR factorization $Y_j = Q_jR_j$ \label{alg_rsi_second_qr}
      \EndFor
      \State $Q \gets Q_q$
      \State \textbf{return} $Q$
    \EndProcedure
  \end{algorithmic}
\end{algorithm}

We modify \ALG{alg:original_randomized_subspace_iteration} in such a way that it estimate the orthonormal basis matrix $Q$ for $\mathscr{X}=X - E\mathbf{1}_n^T$ from the $m \times n$ matrix $X$ and the $m$ dimensional vector $E$ without explicitly forming $\mathscr{X}$.
\ALG{alg:randomized_subspace_iteration} is the modified version of the randomized subspace iteration algorithm. 
The modifications are in two folds.
First, the power matrix $Y$ is approximated using only one $QR$ factorization at each iteration of the algorithm as opposed to original version that uses two $QR$ factorizations. 
We change the factorization in \EQ{eq:pow_qr1} to \EQ{eq:pow_qr2}.
\begin{equation}
  Q_{q}(\prod_{i=0}^{q-1} R_{q-i})R_0 = (XX^T)^qX\Omega 
  \label{eq:pow_qr2}
\end{equation}
where $Q_0R_0 = X\Omega$, and $Q_iR_i=X(X^TQ_{i-1})$.
Note that the product $X(X^TQ_{i-1})$ can be rapidly computed if higher priority is given to the right-hand side product as it is shown by the parenthesis. 
Second, we add one extra step to the algorithm that updates the QR factorization of $Y$ with respect to the input vector $E$ such that $\mathscr{X} \approx QQ^T\mathscr{X}$, where $\mathscr{X}=X - E\mathbf{1}_n^T$. 
The step is done in Line~\ref{alg:randomized_subspace_iteration:qrupdate} using the QR-update algorithm described by \namecite[p.~607]{Golub:MC}. 
For a given QR factorization such as $QR=Y$ and two vectors $u$, and $v$, the QR-update algorithm compute the QR-factorization of $Q'R'=Y+uv^T$ through updating the already available factors $Q$ and $R$. 
Using this algorithm, we can compute the basis matrix of the mean centred matrix $\mathscr{X}$ without explicitly building the matrix. 
%Moreover, for a given $m\times n$ matrix, the algorithm runs is $O(N^2)$ time complexity, where $N=\mbox{max}(m,n)$, which is faster that computing QR factorization from scratch running in $O(N^3)$. 
\begin{algorithm}[H]
  \caption{Estimating the orthonormal basis matrix $Q$ for $\mathscr{X}=X-E\mathbf{1}_n^T$, where $X$ is an $m \times n$ matrix, $E$ is an $m$ dimensional vector and  $\mathbf{1}_n$ is an $n$ dimensional vector of ones.}
  \label{alg:randomized_subspace_iteration}
  \begin{algorithmic}[1]
    \Procedure{Centred-Randomized-Range-Finder}{$X,E,K,q$} 
      \State Draw an $n \times K$ standard Gaussian matrix $\Omega$ 
      \State Form $Y_0 \gets X\Omega$ and compute the QR factorization $Y_0 = Q_0R_0$
      \For {$j\gets1$ \textbf{to} $q$}
        \State Form $Y_j \gets X (X^TQ_{j-1})$ and compute the QR factorization $Y_j = Q_jR_j$
      \EndFor
      \State Compute the QR factorization $QR = Q_qR_q - E\mathbf{1}_n^T$ using the QR update algorithm \cite{Golub:MC} \label{alg:randomized_subspace_iteration:qrupdate}
      \State \textbf{return} $Q$
    \EndProcedure
  \end{algorithmic}
\end{algorithm}


==> union_eigenvalues.tex <==
\begin{figure}
  \begin{center} 
    \subfloat[]{\scalebox{0.6} {
        \label{subfig:left_union_eigenvalue}
        \input{left_union_context_eigval.tex}
      }
    }
    \hfill
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \subfloat[]{\scalebox{0.6} {
        \label{subfig:right_union_eigenvalue}
        \input{right_union_context_eigval.tex}
      }
    }
    \hfill
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \subfloat[]{\scalebox{0.6} {
        \label{subfig:symmetric_union_eigenvalue}
        \input{symmetric_union_context_eigval.tex}
      }
    }

  \end{center}
  \caption{The spectrum of eigenvalues obtained from covariance matrices of principal word vectors generated with (a) the backward union context, (b) the forward union context, and (c) the symmetric union context. The vertical axes are the logarithm of the eigenvalues.}
  \label{fig:union_eigenvalues}
\end{figure}



==> union_sim_rank.tex <==
\begin{figure}[htp]
  \begin{center} 
    \subfloat[]{\scalebox{1} {
      \label{subfig:backward_union_sim_rank}
      \input{left_union_context_sim_rank.tex}
    }
  }
  \vfill
  \subfloat[]{\scalebox{1} {
      \label{subfig:forward_union_sim_rank}
      \input{right_union_context_sim_rank.tex}
    }
  }
  \vfill
  \subfloat[]{\scalebox{1} {
      \label{subfig:symmetric_union_sim_rank}
      \input{symmetric_union_context_sim_rank.tex}
    }
  }
  \end{center}

  \caption{ {\bf a}: the best spectrum of eigenvalues obtained from different families of feature variables. Vertical axis is the logarithm of eigenvalues. {\bf b}: the logarithm of the generalized variance of the the princiapl word vectors obtained from different types of feature variables. neighbourhood: $\mathbf{F}(F,\mathscr{C}_n^{\abs{\tau}=1})$; asym-window: $\mathbf{F}(F,\mathscr{C}_{\{f,b\}w}^{k=10})$; sym-window: $\mathbf{F}(F,\mathscr{C}_{sw}^{K=3})$; left-union: $\mathbf{F}(F,\mathscr{C}_{u}) = \bigcup_{\tau=-5}^{-1} \mathbf{F}(F,\mathscr{C}_n^{\tau})$; right-union: $\mathbf{F}(F,\mathscr{C}_{u}) = \bigcup_{\tau=1}^{5} \mathbf{F}(F,\mathscr{C}_n^{\tau})$; dependency: $\mathbf{F}(F,\mathscr{C}_d)$}
  \label{fig:best_eigenval}
\end{figure}



==> window_based_eigenvalues.tex <==
\begin{figure}
  \begin{center} 
    \subfloat[]{\scalebox{0.6} {
        \label{subfig:left_window_eigenvalue}
        \input{left_window_context_eigval.tex}
      }
    }
    \hfill
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \subfloat[]{\scalebox{0.6} {
        \label{subfig:right_window_eigenvalue}
        \input{right_window_context_eigval.tex}
      }
    }
    \hfill
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
     \subfloat[]{\scalebox{0.6} {
        \label{subfig:symmetric_window_eigenvalue}
        \input{symmetric_window_context_eigval.tex}
      }
    }
    %\vfill
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    %\subfloat[]{\scalebox{0.6} {
    %    \label{subfig:left_union_eigenvalue}
    %    \input{left_union_context_eigval.tex}
    %  }
    %}
    %\hfill
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    %\subfloat[]{\scalebox{0.6} {
    %    \label{subfig:right_union_eigenvalue}
    %    \input{right_union_context_eigval.tex}
    %  }
    %}
    %\hfill
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    %\subfloat[]{\scalebox{0.6} {
    %    \label{subfig:symmetric_union_eigenvalue}
    %    \input{symmetric_union_context_eigval.tex}
    %  }
    %}

  \end{center}
  \caption{The spectrum of eigenvalues obtained from covariance matrices of principal word vectors generated with (a) the backward window-based context, (b) the forward window-based context, and (c) the symmetric window-based context. The vertical axes are the logarithm of the eigenvalues.}
  \label{fig:window_based_eigenval}
\end{figure}



==> window_based_sim_rank.tex <==
\begin{figure}[htp]
  \begin{center} 
    \subfloat[]{\scalebox{1} {
      \label{subfig:backward_window_sim_rank}
      \input{left_window_context_sim_rank.tex}
    }
  }
  \vfill
  \subfloat[]{\scalebox{1} {
      \label{subfig:forward_window_sim_rank}
      \input{right_window_context_sim_rank.tex}
    }
  }
  \vfill
  \subfloat[]{\scalebox{1} {
      \label{subfig:symmetric_window_sim_rank}
      \input{symmetric_window_context_sim_rank.tex}
    }
  }
  \end{center}
  \label{fig:window_based_sim_rank}
\end{figure}



==> word_form_fisher.tex <==
\begin{figure}[htp]
  \begin{center}
    \subfloat[]{\scalebox{0.57} {
      \input{word_form_neighbourhood_syntactic_fisher.tex}
      \label{subfig:word_form_neighbourhood_syntactic_fisher}
      }
    }
    %
    \hfill
    %
    \subfloat[]{\scalebox{0.57} {
      \input{word_form_window-based_syntactic_fisher.tex}
      \label{subfig:word_form_window-based_syntactic_fisher}
      }
    }
    %\hspace{0.2\textwidth} %\hfill
    \hfill
    \subfloat[]{\scalebox{0.57} {
      \input{word_form_union_syntactic_fisher.tex}
      \label{subfig:word_form_union_syntactic_fisher}
      }
    }
    %
    \vfill
    %
    \subfloat[]{\scalebox{0.57} {
      \input{word_form_ner_neighbourhood_fisher.tex}
      \label{subfig:word_form_ner_neighbourhood_fisher}
      }
    }
    %
    \hfill
    %
    \subfloat[]{\scalebox{0.57} {
      \input{word_form_ner_window-based_fisher.tex}
      \label{subfig:word_form_ner_window-based_fisher}
      }
    }
    %\hspace{0.2\textwidth} %\hfill
    \hfill
    \subfloat[]{\scalebox{0.57} {
      \input{word_form_ner_union_fisher.tex}
      \label{subfig:word_form_ner_union_fisher}
      }
    }
  \end{center}
  \caption{Fisher discriminant ratio (FDR) of principal word vectors with regard to word's part of speech tags (top) and named entities (bottom). The word vectors are extracted different types of features variables formed with word forms and (a,d) neighbourhood context, (b,e) window-based context, (c,f) union context.}
  \label{fig:word_form_fisher}
\end{figure}



==> word_variables.tex <==
\subsection{Word Variables}
\label{subsec:word_variables}
As before, we denote a corpus as $E=\{e_1,\dots,e_T\}$ and refer to each element $e_i\in E$ ($i=1,\dots,T$) as a \emph{token}.
Each token in $E$ is a sequence of characters. 
We define a vocabulary set as a set of clusters over the tokens in a corpus. 
Given a vocabulary set, we associate each token cluster with a random variable called \emph{word variable} indicating whether a token $e_i\in E$ is part of the cluster or not. 

The tokens can be clustered in different ways. 
It is usually done on the basis of character sequences forming the tokens or the distribution of tokens in the corpus. 
In the most simplest way, we put the tokens with the same sequences of characters in the same clusters.  
Due to the Zipfian distribution of the words, this approach results in a large number of clusters that most of them contains a few tokens. 
Some remedies to this problem are as follows.
In the languages that have both upper-case and lower-case letters (e.g. Germanic languages such as English, and Swedish), it is common to merge the clusters of tokens that have the same sequences of letters without regard to the form of the letter. 
This approach is equivalent with replacing all letters in the corpus with their lower-case forms. 
It is also quite common to merge those cluster with small number of tokens into a single cluster and use a single word variable for all of them.
This word variable is called the \emph{unknown} word variable since it indicates the words will small frequencies. 
This is equivalent with replacing less frequent tokens in the corpus with the special token \emph{unknown}.
Alternatively, one can cluster the tokens with respect to their lemmas or stems. 
This approach is expected to dramatically reduces the size of the vocabulary set and be helpful for the cases where the inflectional forms of the words are not of interest. 
One might also want to put all tokens that follow a specific pattern into a cluster. 
For example, we usually put the sequences of digits into a same cluster and associate it with a single word variable called \emph{number}. 


